Towards Large-scale Chemical Reaction Image Parsing via a Multimodal Large Language Model

Artificial intelligence (AI) has demonstrated significant promise in advancing organic chemistry research; however, its effectiveness depends on the availability of high-quality chemical reaction data. Currently, most published chemical reactions are not available in machine-readable form, limiting the broader application of AI in this field. The extraction of published chemical reactions into structured databases still relies heavily on manual curation, and robust automatic parsing of chemical reaction images into machine-readable data remains a significant challenge. To address this, we introduce the Reaction Image Multimodal large language model (RxnIM), the first multimodal large language model specifically designed to parse chemical reaction images into machine-readable reaction data. RxnIM not only extracts key chemical components from reaction images but also interprets the textual content that describes reaction conditions. Together with specially designed large-scale dataset generation method to support model training, our approach achieves excellent performance, with an average F1 score of 88% on various benchmarks, surpassing literature methods by 5%. This represents a crucial step toward the automatic construction of large databases of machine-readable reaction data parsed from images in the chemistry literature, providing essential data resources for AI research in chemistry. The source code, model checkpoints, and datasets developed in this work are released under permissive licenses. An instance of the RxnIM web application can be accessed at https://huggingface.co/spaces/CYF200127/RxnIM.

==> figures/algri.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=1\textwidth]{figures/algri1.pdf}
c\caption{Overall pipeline of our Synthetic Image Generation Algorithm. We first generate the reaction components from the pistachio dataset. Then we synthetic several sub-images using the reaction components based on the pre-defined reaction pattern. The final synthetic reaction image is obtained by combining and post-processing the sub-images.}                          
\label{fig:algri}
\end{figure*}

==> figures/img_example.tex <==
\begin{figure*}[h]
\centering
\includegraphics[width=1\textwidth]{figures/img_example1.pdf}
\caption{Examples of reaction images in chemical literature. We divide the reaction images into four patterns: single-line, multiple-line, branch, and cycle.}                          
\label{fig:img_example}
\end{figure*}


==> figures/matrix.tex <==
\begin{figure*}[h]
\centering
\includegraphics[width=1\textwidth]{figures/matrix.png}
\caption{Confusion matrix of the OCR and role identification task(Normalized by true labels).}                          
\label{fig:matrix}
\end{figure*}


==> figures/model.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=1\textwidth]{figures/model1.pdf}
\caption{Overall architecture of our ReactionImgMLLM. The model incorporates four key components: 
1) A unified language-based task instruction that standardizes the interface for defining and customizing tasks related to image-based chemical reaction data extraction.
2) A multimodal encoder that aligns reaction image information with task instructions to generate task-aware image features.
3) A task-guided ReactionImg tokenizer that converts these features into image tokens based on task instructions.
4) An open-ended LLM task decoder that uses the image tokens and language instructions to generate the final outputs.}                          
\label{fig:model}
\end{figure*}


==> figures/parsing.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=1\textwidth]{figures/parsing.pdf}
\caption{Illustration of the output-format-as-query decoding strategy. Format 1 denotes the desired output format of the reaction extraction task as mentioned in Sec.~\ref{sec:Reaction Extraction Task}. Format 2 denotes the desired output format of the condition OCR and role identification task  as mentioned in Sec.~\ref{sec:Condition OCR and Role Identification Task}.}                          
\label{fig:parsing}
\end{figure*}

==> tables/dataset.tex <==
\begin{table}[h]
  \centering
  \caption{\textbf{Statistics of different datasets for image-based reaction parsing tasks.} We provide a detailed breakdown of the synthetic and real datasets, including the number of samples used for training, validation, and testing across the two main tasks: reaction component identification task and reaction condition interpretation task. The conventional object detection task data is used in the synthetic dataset but is not shown here since it's not included in the reaction parsing tasks.}
  \begin{tabular}{@{}cccccc@{}}
    \toprule
    Dataset & Task & Train Sample & Valid Sample & Test Sample \\
    \midrule
    \multirow{2}{*}{Synthetic} & Reaction Component Identification  & 48160 & 6020 & 6020 \\
    &  Reaction Condition Interpretation & 166116 & 20765 & 20764 \\
    \midrule
    \multirow{2}{*}{Real} & Reaction Component Identification  & 1240 & 138 & 138 \\
    &  Reaction Condition Interpretation & -- & -- & -- \\
    \bottomrule
  \end{tabular}
  %\footnotetext{We provide a detailed breakdown of the synthetic and real datasets, including the number of samples used for training, validation, and testing across the two main tasks: reaction extraction and condition OCR \& role identification. The conventional object detection task data is used in the synthetic dataset but is not shown here since it's not included in the reaction parsing tasks.}
\label{tab:dataset}
\end{table}


==> tables/role.tex <==
\begin{table}[h]
  \centering
  \caption{Accuracy of the OCR and Role Identification Task. Scores are in \%.}
  \label{tab:ocr_role_id}
  \begin{tabular}{@{}lcc@{}}
    \toprule
    Model            & OCR Accuracy (\%) & CRI Accuracy (\%) \\
    \midrule
    ReactionImgMLLM  & 94.91             & 93.62                             \\
    \bottomrule
  \end{tabular}
\end{table}

==> tables/tab_abl_location.tex <==
\begin{table}[ht]
  \centering
  \caption{Ablation Studies on Different Position Representations.}
  
  \begin{tabular}{lccc}
    \toprule
    Position Representation & Precision & Recall &  F1 \\
    \midrule
    \multicolumn{1}{c}{Vocab} & 86.15 & 81.23 & 83.62 \\
    \multicolumn{1}{c}{Numerical} & \textbf{86.91} & \textbf{82.77} & \textbf{84.79} \\
    \bottomrule
  \end{tabular}
  \label{tab:position}
\end{table}

==> tables/tab_abl_sep.tex <==
\begin{table}[h]
  \centering
  \caption{Ablation Studies on Different Training Strategies.}
  \renewcommand\arraystretch{1.2}
  \setlength{\tabcolsep}{5pt}
  \begin{tabular}{@{}ccccccc@{}}
    \toprule
    \multirow{2}{*}{Joint Training} & \multicolumn{3}{c}{Reaction Extraction Task} & \multicolumn{2}{c}{OCR and Role Identification Task} \\
    \cmidrule(lr){2-4} \cmidrule(lr){5-6}
     & Precision & Recall & F1 & OCR Accuracy & CRI Accuracy \\
    \midrule
    \xmark & 86.84 & 82.64 & 84.68 & 94.78 & 93.39 \\
    \cmark   & \textbf{86.91} & \textbf{82.77} & \textbf{84.79} & \textbf{94.91} & \textbf{93.62} \\
    \bottomrule
  \end{tabular}
  \label{tab:abl_sep}
\end{table}



==> tables/tab_abl_textencoder.tex <==
\begin{table}[t]
  \centering
  \caption{Ablation Studies on the Effect of Text Encoder.}
  \label{tab:textencoder}
  \renewcommand\arraystretch{1.2}
  \setlength{\tabcolsep}{5pt}
  \begin{tabular}{ccccccc}
    \toprule
    \multirow{1}{*}{w/BERT} & \multirow{1}{*}{Freeze} & \multicolumn{3}{c}{Reaction Extraction Task} & \multicolumn{2}{c}{OCR and Role Identification Task} \\
    \cmidrule(lr){3-5} \cmidrule(lr){6-7}
     &  & Precision & Recall & F1 & OCR Accuracy & CRI Accuracy \\
    \midrule
    \xmark & \xmark & \underline{82.21} & \underline{78.55} & \underline{80.34} & \underline{94.74} & \underline{93.41} \\
    \cmark & \xmark & \textbf{86.91} & \textbf{82.77} & \textbf{84.79} & \textbf{94.91} & \textbf{93.62} \\
    \cmark & \cmark & 71.65 & 70.02 & 69.10 & 94.21 & 81.73 \\ % Assume these values are second best, modify if needed
    \bottomrule
  \end{tabular}
\end{table}

==> tables/tab_abl_tokens.tex <==
\begin{table}[t]
  \centering
  \caption{Ablation studies on Different Numbers of Image Tokens.}
  \renewcommand\arraystretch{1.2}
  \setlength{\tabcolsep}{5pt}
  \begin{tabular}{@{}ccccccc@{}}
    \toprule
    \multirow{2}{*}{Number of Image Tokens} & \multicolumn{3}{c}{Reaction Extraction Task} & \multicolumn{2}{c}{OCR and Role Identification Task} \\
    \cmidrule(lr){2-4} \cmidrule(lr){5-6}
     & Precision & Recall & F1 & OCR Accuracy & CRI Accuracy \\
    \midrule
    100 & 85.62 & 82.11 & 83.83 & 93.68 & 92.85 \\
    200 & 86.31 & \underline{82.36} &\underline{84.29} & 94.26 & 93.02 \\
    300 & \textbf{86.91} & \textbf{82.77} & \textbf{84.79} & \underline{94.91} & \textbf{93.62} \\
    400 & \underline{86.42} & 82.20 & 84.26 & \textbf{95.02} & \underline{93.14} \\
    \bottomrule
  \end{tabular}
  \label{tab:tokens}
\end{table}

==> tables/tab_sota_sys.tex <==
\begin{table}[h]
  \centering
  \caption{ Comparison of Model Performance on the Reaction Data Extraction Task on the Synthetic Test Set. Scores are in \%.}
 
  \label{tab:performance_comparison_sys}
  \renewcommand\arraystretch{1.2}
  \setlength{\tabcolsep}{5pt}
  \begin{tabular}{@{}cccccccc@{}}
    \toprule
    \multirow{2}{*}{Model} & \multicolumn{3}{c}{Hard Match} & \multicolumn{3}{c}{Soft Match} \\
    \cmidrule(lr){2-4} \cmidrule(lr){5-7} 
     & Precision & Recall & F1 & Precision & Recall & F1 \\
    \midrule
    ReactionDataExtractor~\cite{3wilary2021reactiondataextractor} & 8.40 & 6.90 & 7.60 & 22.60 & 11.40 & 15.20 \\
    OChemR~\cite{OChemR} & 8.10 & 7.50 & 7.80 & 15.90 & 12.80 & 14.20 \\
    RxnScribe~\cite{5qian2023rxnscribe} & \underline{78.54} & \underline{75.63} & \underline{77.06} & \underline{87.62} & \underline{83.95} & \underline{85.75} \\
    ReactionImgMLLM & \textbf{86.41} & \textbf{85.92} & \textbf{86.16} & \textbf{91.55} & \textbf{90.81} & \textbf{91.18} \\
    \bottomrule
  \end{tabular}
\end{table}

